Holmes: Towards Distributed Training Across Clusters with Heterogeneous NIC Environment

Large language models (LLMs) such as GPT-3, OPT, and LLaMA have demonstrated remarkable accuracy in a wide range of tasks. However, training these models can incur significant expenses, often requiring tens of thousands of GPUs for months of continuous operation. Typically, this training is carried out in specialized GPU clusters equipped with homogeneous high-speed Remote Direct Memory Access (RDMA) network interface cards (NICs). The acquisition and maintenance of such dedicated clusters is challenging. Current LLM training frameworks, like Megatron-LM and Megatron-DeepSpeed, focus primarily on optimizing training within homogeneous cluster settings. In this paper, we introduce Holmes, a training framework for LLMs that employs thoughtfully crafted data and model parallelism strategies over the heterogeneous NIC environment. Our primary technical contribution lies in a novel scheduling method that intelligently allocates distinct computational tasklets in LLM training to specific groups of GPU devices based on the characteristics of their connected NICs. Furthermore, our proposed framework, utilizing pipeline parallel techniques, demonstrates scalability to multiple GPU clusters, even in scenarios without high-speed interconnects between nodes in distinct clusters. We conducted comprehensive experiments that involved various scenarios in the heterogeneous NIC environment. In most cases, our framework achieves performance levels close to those achievable with homogeneous RDMA-capable networks (InfiniBand or RoCE), significantly exceeding training efficiency within the pure Ethernet environment. Additionally, we verified that our framework outperforms other mainstream LLM frameworks under heterogeneous NIC environment in terms of training efficiency and can be seamlessly integrated with them.

==> hetnet.tex <==
\begin{figure*}
  \centering
  \includegraphics[width = 0.86\textwidth]{figs/example_normal.pdf}
  \caption{An illustration of parallelism mechanism in Holmes. In this case, a transformer-based model with 6 layers is trained across 2 clusters. Each cluster comprises 2 nodes, each equipped with 4 GPU devices. Communication between Node 1 and Node 2 utilizes InfiniBand, while Node 3 and Node 4 use RoCE. However, there is no high-speed interconnect between the two clusters, and communication between them relies solely on low-speed Ethernet. For parallelism settings, the degrees of data, tensor, and pipeline parallelisms are 2, 2, and 4, respectively. Pipeline parallelism is implemented between the two clusters using Ethernet. The model's layers are unevenly partitioned into 2 stages and further distributed to different GPU devices. Data parallelism is performed within each cluster using RDMA, and tensor parallelism is implemented within each node using NVLink.}
  % \caption{An illustration of parallelism mechanism in Holmes: A 6-layer transformer model is trained across 2 clusters, each with 2 nodes equipped with 4 GPUs. Communication between Node 1 and Node 2 uses InfiniBand, and Node 3 and Node 4 use RoCE. However, there's no high-speed interconnect between clusters; communication relies on low-speed Ethernet. For parallelism settings, the degrees of data, pipeline, and tensor parallelisms are 2, 2, and 4, respectively. Pipeline parallelism is implemented between clusters using Ethernet. Model layers are unevenly partitioned into 2 stages and distributed to GPUs in 2 clusters. Data parallelism occurs within each cluster using RDMA, and tensor parallelism is implemented within each node using PCI-E.}
  \label{example}
\end{figure*}

In this section, we present the Holmes design. Holmes is developed within the framework of Megatron-LM~\cite{shoeybi2019megatron,narayanan2021efficient}, a popular tool for LLM training. Our approach re-optimizes two types of parallelism techniques: model parallelism and data parallelism. Model parallelism is further categorized into tensor parallelism and pipeline parallelism.

In distributed training, pipeline parallelism typically has less communication overhead than data parallelism because different GPU devices handle sequential computational stages with less inter-device communication between them~\cite{huang2019gpipe,narayanan2019pipedream}. For data parallelism, data is divided into segments, and each device independently processes a portion. These units simultaneously perform identical operations on separate data, leading to increased communication for synchronization and greater overhead~\cite{rasley2020deepspeed, ren2021zero}. Holmes enhances the built-in communication methods for pipeline and data parallelism in Megatron-LM. Figure~\ref{example} illustrates the parallelism mechanism in Holmes. Further details will be discussed in the subsequent parts.

\subsection{Model Parallelism}
\subsubsection{Tensor Model Parallelism}
Tensor model parallelism involves distributing individual layers of the model across multiple GPU devices. In the tensor parallelism of our framework, different layers of the model are assigned to various GPU devices within the same node, enabling concurrent processing of these layers, and thereby accelerating the training process. As a result, the communication operations associated with tensor parallelism predominantly take place within the same node, leveraging technologies such as PCI-E~\cite{kaldewey2012gpu, li2019evaluating} or NVLink~\cite{foley2017ultra} to facilitate inter-device communication.

Holmes adopts the same partitioning strategy used by Megatron-LM for transformer layers, which serve as the fundamental components of LLMs~\cite{narayanan2021efficient}.
Following the partitioning process, we obtain the tensor parallel matrix denoted as $[\textbf{TP}]\in \mathbb{Z}_{+}^{(p\ \cdot\ d) \times t}$. This matrix contains various parallel groups, and the GPU devices within each group belong to the same node. We represent $[\textbf{TP}]_{i,j}$ as the $j$-th device in the $i$-th tensor parallel group, which can be formalized as follows:
\begin{equation}
\label{eq:tp}
{[\textbf{TP}]_{i,j} = \operatorname{rank}_{(i-1) \cdot t + j}}\quad_{j \in \{1,2\ ,...,\ t\}}^{i \in \{1,2\ ,...,\ p\ \cdot\ d\}}
\end{equation}

Due to space limitations, we omit the further technical introduction in this section. For more detailed information on tensor parallelism, refer to~\cite{narayanan2021efficient}.

% In these matrices, $[\textbf{PP}]_{i,j}$ denotes the $j$-th device in the $i$-th pipeline parallel group, $[\textbf{TP}]_{i,j}$ denotes the $j$-th device in the $i$-th tensor parallel group, and $[\textbf{DP}]_{i,j}$ signifies the $j$-th device in the $i$-th data parallel group.

\subsubsection{Pipeline Model Parallelism}
In traditional pipeline parallelism, the model layers are segmented into different computational stages, each assigned to different GPU devices. These devices execute the stages sequentially, transferring their results to subsequent stages. Communication operations occur through the exchange of data between these devices. When dealing with models that contain repeated transformer blocks, each GPU device can effectively manage an equal number of these blocks. This process involves breaking a batch into smaller micro-batches and executing them in a pipeline fashion~\cite{huang2019gpipe,narayanan2019pipedream,narayanan2021memory}. 
% This pipelining strategy ensures that inputs maintain a consistent view of weight versions during both forward and backward passes, ensuring well-defined synchronous weight updates. 
We use periodic pipeline flushes to maintain the synchronization of optimizer steps between GPU devices.

% Specifically, when one computational stage is completed, it passes the generated data to the next computational stage. This often involves sending data to the next device through a network or other communication channel so that subsequent computational stages can use these data. This data transfer and communication are integral parts of pipeline parallelism, ensuring that different parts of the model work together correctly throughout the training process. This helps improve training efficiency, reduce communication overhead, and improve the effectiveness of distributed training.

The implementation of our pipeline parallelism is similar to PipeDream-Flush~\cite{narayanan2021memory}. To support LLM training across clusters equipped with heterogeneous NICs, we make the following innovative improvements.

\paragraph{Cross-Cluster Pipeline Parallelism.} Current LLM training frameworks exclusively support LLM training with low-speed Ethernet NICs within clusters that possess heterogeneous NICs. To address these limitations, we have introduced a solution to enable LLM training in the heterogeneous NIC environment. Capitalizing on the relatively low communication cost of pipeline parallelism, we establish pipeline parallelism groups among multiple clusters that lack high-speed interconnects. Consequently, these pipeline parallelism groups consist of GPU devices connected via heterogeneous NICs, and their sole means of communication is through Ethernet due to NIC incompatibility. Conversely, owing to the division of pipeline parallelism groups, the data parallelism groups can comprise GPU devices connected via homogeneous NICs, enabling communication via RDMA NICs. In terms of tensor parallelism, it is confined to the same node and communicates via PCI-E or NVLink interfaces.
\begin{table}
    \begin{center}
    \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{lccc}
    \hline
    \textbf{NIC Env} & \textbf{TFLOPS} & \textbf{Throughtput} & \textbf{Bandwidth (Gbps)} \\ \hline
    % InfiniBand & 197 & 99.23 & 66.0  \\ 
    % RoCE       & 160 & 80.54 & 45.6  \\ 
    % Ethernet   & 122 & 61.32 &  -    \\ \hline
    InfiniBand & 197 & 99.23 & 200  \\ 
    RoCE       & 160 & 80.54 & 200  \\ 
    Ethernet   & 122 & 61.32 & 25   \\ \hline
    \end{tabular}
    }
    \caption{Comparison of TFLOPS and Throughput metrics when training a GPT model with 3.6 billion parameters on 4 nodes using InfiniBand, RoCE, and Ethernet respectively. Each node is equipped with 8 NVIDIA A100 GPUs. We also list the bandwidth of different NICs in the 3rd column.}
    \label{t1}
    \end{center}
\end{table}
Considering that data parallelism relies more on high-speed RDMA NICs than pipeline parallelism does, our Cross-Cluster Pipeline Parallelism method significantly enhances LLM training performance by scheduling pipeline parallelism groups across different clusters in heterogeneous NIC environments.

\paragraph{Self-Adapting Pipeline Partition.} Traditional pipeline parallelism was initially designed for training LLM in the homogeneous NIC environment. In such settings, the model layers are uniformly divided into different stages, ensuring relatively equal computational speeds across various stages of pipeline parallelism. This uniform partitioning is considered the most suitable choice, as all GPU devices exhibit equal computational speeds~\cite{narayanan2021efficient}. However, in the context of a heterogeneous NIC environment, different GPU devices may demonstrate varying computational speeds due to the diverse NICs to which they are connected. Table~\ref{t1} presents a comparison of GPU performance using three different types of NIC during LLM training. Even if InfiniBand and RoCE NICs have the same bandwidth, the GPU device equipped with different types of NIC may exhibit significant variations in actual computational speed (TFLOPS). The observed disparities in TFLOPS and Throughput metrics underscore the inadequacy of a straightforward uniform partition for pipeline parallelism in the heterogeneous NIC environment.

In response to this challenge, we have developed a self-adaptive pipeline partitioning strategy that takes into consideration the specific NIC connected to each GPU device. This strategy optimizes the training process in the heterogeneous NIC environment by distributing varying numbers of layers in the model to different devices based on their connected NIC. To formalize the Self-Adapting Pipeline Partition strategy, we define the computational speed of a device within InfiniBand and RoCE as $S(\textsc{IB})$ and $S(\textsc{RoCE})$, respectively, interpreted as TFLOPS. Assuming a pipeline parallelism group with two devices connected to different NICs and a total number of layers for the model denoted as $N$, the number of layers distributed to the device connected to the InfiniBand NIC (denoted as $N_{ib}$) is calculated as follows:
\begin{equation}
\label{eq:self-pp}
N_{ib} = \lfloor \frac{\alpha \cdot S(\textsc{IB})}{S(\textsc{IB}) + S(\textsc{RoCE})} \cdot N \rfloor 
\end{equation}
where $\alpha$ is the hyper-parameter. $N_{roce}$ can be directly obtained by subtracting $N_{ib}$ from $N$.It can be easily extended to scenarios where the pipeline parallel size is more than 2. Our objective is to allocate a greater number of model layers to the GPU device connected to the faster NIC.
% Similarly, the calculation of $N_{roce}$ follows the same method, ensuring $N_{ib} + N_{roce} = N$.
\paragraph{Summary.}
We introduce two innovative enhancements to pipeline parallelism: optimizing communication operations and adapting to the heterogeneous NIC environment. We illustrate the process with a case presented in Figure~\ref{example}.

To formalize the process of pipeline parallelism, we represent $[\textbf{PP}]_{i,j}$ as the $j$-th device in the $i$-th pipeline parallel group, which can be formalized as follows:
\begin{equation}
\label{eq:pp}
{[\textbf{PP}]_{i,j} = \operatorname{rank}_{i + (j-1) \cdot t \cdot d }}\quad_{j \in \{1,2\ ,...,\ p\}}^{i \in \{1,2\ ,...,\  t\ \cdot\ d\}}
\end{equation}
The formulation is applicable to both homogeneous and heterogeneous NIC environments. In the heterogeneous environment, $[\textbf{PP}]_{i,*}$ represents the $i$-th pipeline parallel group comprising $p$ GPU devices that are connected to different types of NIC.

\subsection{Data Parallelism}
In traditional data parallelism, each GPU device possesses a complete replica of the model, while the input dataset is partitioned among these GPU devices. Periodically, these GPU devices synchronize their gradients to maintain consistent model weights across all of them. In cases where the model is too large to fit within a single worker, data parallelism is often used in conjunction with tensor and pipeline parallelism. In this scenario, data parallelism is applied to the smaller model segments that result from the process of model parallelism. The primary advantage of data parallelism lies in its ability to scale deep learning training, allowing the processing of larger datasets in less time. This scalability is particularly beneficial for training LLMs with large datasets.

Communication operations in data parallelism occur in the following steps:
\begin{itemize}[itemsep=1pt,topsep=1pt,parsep=1pt]
    \item \textbf{Data Partition:} The input dataset is divided into smaller batches, with each batch assigned to a different GPU for processing.
    \item \textbf{Gradient Computationn}: Each GPU computes gradient information to help update the model parameters.
    \item \textbf{Gradient Aggregation}: At the end of each batch or epoch, GPUs use the Ring Allreduce algorithm~\cite{sergeev2018horovod} to share and combine their calculated gradient information. This algorithm circulates gradient details in a circular manner among GPUs, accumulating gradients on each GPU until all receive the global gradient information.
    \item \textbf{Model Update}: After receiving the combined gradient information, all GPUs use it to update the model parameters, ensuring that all GPUs have consistent model versions.
\end{itemize}
Communication between GPUs primarily takes place during the Gradient Aggregation step. This communication is facilitated by high-speed RDMA NIC and libraries like NCCL~\cite{nccl}, ensuring the synchronization of gradients between GPUs and maintaining consistent model parameters across all devices.

\begin{figure}[t]
  \centering
  \fbox{\includegraphics[width = 0.45\textwidth]{figs/code3.pdf}}
  \caption{A code snippet for creating data parallel groups across clusters within the heterogeneous NIC environment.}
  \label{code}
\end{figure}
Similarly to pipeline parallelism, traditional data parallelism also does not take into account the heterogeneous NIC environment, and it can only support using the low-speed Ethernet NIC when training LLMs in the heterogeneous environment. To address the problem and accelerate the data parallelism in both homogeneous and heterogeneous environments, we make the following innovative improvements.
\begin{table*}[htbp]
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Parameter Group\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Parameters (billion)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attention\\ Heads\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Hidden\\ Size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number \\ of Layers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pipeline \\ Parallel Size\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Batch\\ Size\end{tabular}} \\ \hline
1 & \multirow{2}{*}{3.6} & \multirow{4}{*}{32} & \multirow{2}{*}{3072} & \multirow{2}{*}{30} & \multirow{2}{*}{2} & 768 \\ \cline{1-1} \cline{7-7} 
2 &  &  &  &  &  & 1536 \\ \cline{1-2} \cline{4-7} 
3 & \multirow{2}{*}{7.5} &  & \multirow{2}{*}{4096} & \multirow{2}{*}{36} & \multirow{2}{*}{3} & 1536 \\ \cline{1-1} \cline{7-7} 
4 &  &  &  &  &  & 2688 \\ \hline
\end{tabular}%
}
  	\caption{Details of parameter groups for training GPT models ranging from 3.6 billion to 39.1 billion parameters. Since our optimization focuses on data parallelism and pipeline parallelism, without involving tensor parallelism, for Parameter Group 1 to Parameter Group 4, we set the tensor parallel size to 1.}
   %  For Parameter Group 7 and 8, due to the large parameter size of the model, we set the tensor parallel size to 8.
	\label{t2_small}
\end{table*}
\paragraph{Automatic NIC Selection.} We introduce an auto-select strategy by modifying NCCL~\cite{nccl} and Megatron-LM~\cite{megatronlm} to support hybrid setups of NICs, including InfiniBand, RoCE, and Ethernet. Traditional data parallelism establishes a unified communication environment for the all data parallel communication groups, thus making it unsuitable for GPU devices with mixed NICs. In scenarios where a data parallelism group consists of two GPU devices connected to InfiniBand and RoCE NICs, respectively, due to their inherent incompatibility, it is not possible to simultaneously select InfiniBand and RoCE NICs. Consequently, communication between the two devices is limited to Ethernet, failing to fully utilize high-speed NICs. Therefore, traditional data parallelism frequently faces performance bottlenecks, particularly during the Gradient Aggregation step, as it necessitates waiting for all GPU devices to conclude their computations.

As shown in Figure~\ref{code},  our strategy provides functions that create data parallelism groups based on the actual network environment. It establishes independent communication channels for each group of devices, ensuring that GPU devices within the same data parallelism group are connected to the same type of NIC, while different data parallelism groups can select different NICs. Detailed comparative results are presented in the subsequent Experiment section.

% \paragraph{Overlapped Distributed Optimizer.} Building upon recent research~\cite{megatronllamma}, we have incorporated a novel partition strategy for gradients and optimizer states into our LLM training framework. This strategy, known as the \textit{OverlappedDistributedOptimizer}, can be summarized by the following core principles:
% \begin{itemize}[itemsep=1pt,topsep=1pt,parsep=1pt]
% \item Traditional optimizers such as Adam and SGD independently update individual parameter values, making it unnecessary to maintain parameters as complete entities.
% \item Each collective communication operation should transmit a significant amount of data to optimize the utilization of communication bandwidth.
% \item There should be no additional communication overhead or GPU memory copying involved.
% \end{itemize}
% The \textit{OverlappedDistributedOptimizer} presents an effective approach to seamlessly intertwining communication with computation. This strategy maximizes the potential for overlapping and utilizes interconnection bandwidth to its fullest extent, all while avoiding any additional overhead in terms of communication volume. For in-depth technical details, you can refer to~\cite{megatronllamma}. Specifically, the \textit{OverlappedDistributedOptimizer} is orthogonal to our previous optimizations and can be combined to further enhance training efficiency.

\paragraph{Summary.}
We introduce an innovative enhancements to data parallelism: an optimal selection strategy of NICs in the heterogeneous NIC environment. 
We illustrate the process with a case presented in Figure~\ref{example}.

To formalize the process of data parallelism, we represent $[\textbf{DP}]_{i,j}$ as the $j$-th device in the $i$-th data parallel group, which can be formalized as follows:
\begin{equation}
\label{eq:dp}
{[\textbf{DP}]_{i,j} =  \operatorname{rank}_{\operatorname{mod}(i-1, t) + (\operatorname{floor}(\frac{i-1}{t}) \cdot d + j - 1) \cdot t + 1}}\ _{j \in \{1,2\ ,...,\ d\}}^{i \in \{1,2\ ,...,\ p\ \cdot\ t\}}
\end{equation}
where $\operatorname{mod}(i-1, t)$ denotes the modulo operation, which calculates the remainder when dividing two numbers, and $\operatorname{floor}(*)$ is used to signify rounding down a real number.


